Neural Target Speech Extraction: An Overview

Humans can listen to a target speaker even in challenging acoustic conditions that have noise, reverberation, and interfering speakers. This phenomenon is known as the cocktail-party effect. For decades, researchers have focused on approaching the listening ability of humans. One critical issue is handling interfering speakers because the target and non-target speech signals share similar characteristics, complicating their discrimination. Target speech/speaker extraction (TSE) isolates the speech signal of a target speaker from a mixture of several speakers with or without noises and reverberations using clues that identify the speaker in the mixture. Such clues might be a spatial clue indicating the direction of the target speaker, a video of the speaker's lips, or a pre-recorded enrollment utterance from which their voice characteristics can be derived. TSE is an emerging field of research that has received increased attention in recent years because it offers a practical approach to the cocktail-party problem and involves such aspects of signal processing as audio, visual, array processing, and deep learning. This paper focuses on recent neural-based approaches and presents an in-depth overview of TSE. We guide readers through the different major approaches, emphasizing the similarities among frameworks and discussing potential future directions.

==> notations.tex <==
\def\m{m} % microphone index
\def\t{t} % time index
\def\f{f} % frequency index
\def\n{n} % time frame index
\def\tgt{s} % index of target speaker

\def\T{T} % duration of mixture
\def\N{N} % number of frames
\def\I{I} % number of speakers


\def\Z{\mathbf{Z}} % intermediate representation
\def\Zmix{\mathbf{Z}_\mix} % intermediate representation mix

\def\Ztgt{\mathbf{Z}_\tgt} % intermediate representation

\def\W{\mathbf{L}} % Transformation





% MIXTURE
\def\mix{y}
\def\mixm[#1]{\mix^\m[#1]}
\def\mixmt{\mix^\m[\t]} % mixture, mic index, time index
\def\mixmvec{\mathbf{\mix}^m} % mixture, mic, all times
\def\mixt{\mix[t]} % mixture, time index, ommiting mic index
\def\mixvec{\mathbf{\mix}} % mixture, all times, ommiting mic index
\def\mixf{Y}
\def\mixfmnf{\mixf^\m[\n,\f]} % mixture STFT, mic index, timefr index, freq index
\def\mixfmmat{\mathbf{\mixf}^\m} % mixture STFT, mic index, all timefr, all freq

\def\mixfnf{\mixf[\n,\f]} % mixture STFT, timefr index, freq index, ommiting mic index
\def\mixfmat{\mathbf{\mixf}} % mixture STFT, all timefr, all freq, ommiting mic index

% SOURCE
\def\src{x}
\def\srcmt[#1]{\src_{#1}^\m[\t]} % source, mic index, time index
\def\srcmvec[#1]{\mathbf{\src}_{#1}^m} % source, mic, all times
\def\srct[#1]{\src_{#1}[t]} % source, ommiting mic index, time index
\def\srcvec[#1]{\mathbf{\src}_{#1}} % source ommiting mic index, all times
\def\srcf{X}
\def\srcfmnf[#1]{\srcf_{#1}^\m[\n,\f]} % source STFT, mic index, timefr index, freq index
\def\srcfmmat[#1]{\mathbf{\srcf}_{#1}^\m} % source STFT, mic index, all timefr, all freq
\def\srcfnf[#1]{\srcf_{#1}[\n,\f]} % source STFT, timefr index, freq index, ommiting mic index
\def\srcfmat[#1]{\mathbf{\srcf}_{#1}} % source STFT, all timefr, all freq, ommiting mic index

% Estimate
\def\estsrc{\hat{\src}}
\def\estsrct[#1]{\estsrc_{#1}[t]} 
\def\estsrcvec[#1]{\hat{\mathbf{\src}}_{#1}}
\def\estsrcmt[#1]{\hat{\mathbf{\srcf}}_{#1}}
\def\estfmnf[#1]{\hat{S}_{#1}^\m[\n,\f]} % mixture STFT, mic index, timefr index, freq index


% Interference
\def\int{i}
\def\intt{\intx[t]} % Interference, time index, ommiting mic index
\def\intmt{\intx^\m[\t]} % Interference, mic index, time index
\def\intmvec{\mathbf{\int}^m} % Interference, mic, all times
\def\intt{\int[t]} % Interference, time index, ommiting mic index
\def\intvec{\mathbf{\int}} % Interference, all times, ommiting mic index
\def\intf{I}
\def\intfmnf{\intf^\m[\n,\f]} % Interference STFT, mic index, timefr index, freq index
\def\intfmmat{\mathbf{\intf}^\m} % Interference STFT, mic index, all timefr, all freq
\def\intfnf{\intf[\n,\f]} % Interference STFT, timefr index, freq index, ommiting mic index
\def\intfmat{\mathbf{\intf}} % Interference STFT, all timefr, all freq, ommiting mic 

% NOISE
\def\nois{v}
\def\noismt{\nois^\m[\t]} % noise, mic index, time index
\def\noismvec{\mathbf{\nois}^m} % noise, mic, all times
\def\noist{\nois[t]} % noise, ommiting mic index, time index
\def\noisvec{\mathbf{\nois}} % noise ommiting mic index, all times
\def\noisf{V}
\def\noisfmnf{\noisf^\m[\n,\f]} % noise STFT, mic index, timefr index, freq index
\def\noisfmmat{\mathbf{\noisf}^\m} % noise STFT, mic index, all timefr, all freq
\def\noisfnf{\noisf[\n,\f]} % noise STFT, timefr index, freq index, ommiting mic index
\def\noisfmat{\mathbf{\noisf}} % noise STFT, all timefr, all freq, ommiting mic index

% CLUES
\def\clue{c}
\def\cluemat{\uppercase{\mathbf{C}}_\tgt}

\def\acluet{\clue_\tgt^{(a)}[t]}
\def\acluevec{\mathbf{c}_\tgt^{(a)}}
\def\acluemat{\mathbf{C}_\tgt^{(a)}}
\def\vcluet{\mathbf{\clue}_\tgt^{(v)}[t]}
\def\vcluemat{\uppercase{\mathbf{C}}_\tgt^{(v)}}

\def\dcluet{\clue_\tgt^{(d)}[t]}
\def\dcluemat{\mathbf{C}_\tgt^{(d)}}

% Embeddings
\def\emb{\mathbf{E}_\tgt}
\def\aemb{\mathbf{E}_\tgt^{(a)}}
\def\vemb{\uppercase{\mathbf{E}}_\tgt^{(v)}}

% Mask
\def\maskmt{\mathbf{M}_\tgt}

% Beamformer coefficients
\def\BF{W}
\def\BFfmnf{\BF^\m[\n,\f]} % mixture STFT, mic index, timefr index, freq index
\def\mixfnfmmat{\mathbf{\mixf}[\n,\f]} % mixture STFT, no mic index, all timefr, all freq
\def\mixfnfmmatTrans{\mathbf{\mixf}^{\mathsf{H}}[\n,\f]} % mixture STFT, no mic index, all timefr, all freq


\def\BFnfmmat{\mathbf{\BF}[\f]} % mixture STFT, no mic index, all timefr, all freq
\def\estfnfmmat{\hat{\mathbf{\srcf}}_\tgt[\n,\f]} % mixture STFT, no mic index, all timefr, all freq
\def\estfnfm{\hat{\srcf}_\tgt[\n,\f]} % mixture STFT, no mic index, all timefr, all freq
% Operators

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\TSE}{TSE}
\DeclareMathOperator{\BSS}{BSS}
\DeclareMathOperator{\Denoise}{Denoise}

\DeclareMathOperator{\clueEnc}{ClueEncoder}

\DeclareMathOperator{\Extractor}{TgtExtractor}
\DeclareMathOperator{\SrcDec}{SrcDecoder}
\DeclareMathOperator{\MixEnc}{MixEncoder}
\DeclareMathOperator{\MixNet}{MixNet}
\DeclareMathOperator{\FE}{FE}
\DeclareMathOperator{\VFE}{VFE}
\DeclareMathOperator{\Fusion}{Fusion}
\DeclareMathOperator{\CE}{CE}
\DeclareMathOperator{\InferNet}{InferNet}
\DeclareMathOperator{\Reconstruct}{Reconstruct}
\DeclareMathOperator{\MaskNet}{MaskNet}

\DeclareMathOperator{\NN}{NN}
\DeclareMathOperator{\upsample}{Upsample}
